Grzegorczyk and Whitehead points: the story continues

One of the main goals of region-based theories of space is to formulate a geometrically appealing definition of points. The paper is devoted to the analysis of two such seminal definitions: Alfred N. Whitehead's (1929) and Andrzej Grzegorczyk's (1960). Relying on the work of Loredana Biacino's and Ginagiacomo Gerla's (1996), we improve their results, solve some open problems concerning the mutual relationship between Whitehead and Grzegorczyk points, and put forward open problems for future investigation.

==> basic_mac.tex <==


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{remark}
\newtheorem*{convention}{Convention}%[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{problem}{Problem}
\newtheorem{example}{Example}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{exercise}{Exercise}[section]

%---------------------------------Arrows-------------------------------

\newcommand\Rarrow{\Rightarrow}
\newcommand\Larrow{\Leftarrow}
\newcommand\Iff{\Leftrightarrow}
\newcommand\rarrow{\rightarrow}
\newcommand\larrow{\leftarrow}
\renewcommand\iff{\longleftrightarrow}
\newcommand\fun{\ensuremath{\longrightarrow}}

\newcommand\inj{\stackrel{1-1}{\longrightarrow}}
\newcommand\surj{\stackrel{\text{na}}{\longrightarrow}}
\newcommand\bij{\rightleftarrows}

%---------------------------------Sets of numbers-------------------------------

\newcommand\Real{\varmathbb{R}} %requires txfonts or an external file
\newcommand\Nat{\varmathbb{N}}
\newcommand\Rat{\varmathbb{Q}}
\newcommand\Irr{\varmathbb{I}}
\newcommand\Intgr{\varmathbb{Z}}

\DeclareMathOperator{\Fin}{Fin}


\newcommand{\Even}{\varmathbb{E}} %the set of even numbers
\newcommand{\Odd}{\varmathbb{O}} %the set of odd numbers
\DeclareMathOperator{\lcm}{lcm}  %the least common factor

%---------------------------------Power set-------------------------------

\newcommand{\power}{\mathcal{P}} %power set
\newcommand{\powerne}{\power_{\!+}} %power set without the empty set


%---------------------------------Definitions-------------------------------

%\newcommand\iffdef{\stackrel{\rm df}{\longleftrightarrow}}
\newcommand\iffdef{\;\mathrel{\mathord{:}\mathord{\longleftrightarrow}}\;}
\newcommand\defeq{\coloneqq} %requires mathtools package
\newcommand\eqdef{\eqqcolon}

%---------------------------------Algebras-------------------------------

\newcommand{\zero}{\mathbf{0}} %zero of an algebra
\newcommand{\one}{\mathbf{1}} %unity of an algebra

\newcommand{\ingr}{\sqsubseteq} %part of relation
\newcommand{\ningr}{\not\sqsubseteq} %the complement of part of
\newcommand{\partof}{\sqsubset} %proper part
\newcommand{\overl}{\mathrel{\bigcirc}} %overlap relation
\newcommand{\ext}{\mathrel{\bot}} %incompatibility relation

\newcommand{\Fus}{\mathrel{\mathsf{Fus}}} %mereological fusion relation
\newcommand{\Sum}{\mathrel{\mathsf{Sum}}} %mereological sum relation

\newcommand{\fil}{\mathscr{F}} % a filter
\newcommand{\ult}{\mathscr{U}} % an ultrafilter
\newcommand{\ide}{\mathscr{I}} %an ideal

\DeclareMathOperator{\Ult}{Ult} %all ultrafilters of the algebra
\DeclareMathOperator{\Fil}{Fil} %all filters of the algebra
\DeclareMathOperator{\PFil}{PFil} %all principal filters of the algebra
\DeclareMathOperator{\Gr}{Gr} %all ideals of the algebra
\DeclareMathOperator{\Ide}{Id} %all ideals of the algebra
%\newcommand\Rel{\mathrel{R}} %binary relation
\DeclareMathOperator{\Hom}{Hom} %the collection of all morphisms

\DeclareMathOperator{\CO}{CO} %clopen algebra
\DeclareMathOperator{\RO}{RO} %regular open
\DeclareMathOperator{\RC}{RC} %regular closed

\DeclareMathOperator{\Rego}{R_o} %open regularization
\DeclareMathOperator{\Regc}{R_c} %closed regularization

\newcommand\BA{\boldsymbol{\mathsf{BA}}} %the class of Boolean algebras
\newcommand\BAc{\boldsymbol{\mathsf{BA^c}}} %the class of Boolean contact algebras
\newcommand\BCA{\boldsymbol{\mathsf{BCA}}} %the class of Boolean contact algebras
\newcommand\BCAc{\boldsymbol{\mathsf{BCA^c}}} %the class of complete Boolean contact algebras
\newcommand\BWCA{\boldsymbol{\mathsf{BWCA}}} %the class of Boolean contact algebras
\newcommand\RCA{\boldsymbol{\mathsf{RCA}}} %the class of resolution contact algebras
\newcommand\RCAc{\boldsymbol{\mathsf{RCA^c}}} %the class of complete resolution contact algebras
\newcommand\KTB{\boldsymbol{\mathsf{KTB}}} %the class of KTB modal logics
\newcommand\KTBc{\boldsymbol{\mathsf{KTB^c}}} %the class of complete KTB modal algebras
\newcommand\Cat{\boldsymbol{\mathsf{C}}} %a category

\DeclareMathOperator{\con}{\mathsf{C}} %relacja stycznoci
\DeclareMathOperator{\conk}{\mathsf{K}}
\DeclareMathOperator{\cond}{\mathsf{D}}
\DeclareMathOperator{\Overl}{\mathsf{O}} %the set of all regions that overlap given object


%\usepackage{scalerel,stackengine} is needed for the commands below

%connection relation for filters
\def\twocircs{\mathord{\circ}\!\mathord{\circ}}
\newcommand{\conf}{\mathbin{\twocircs}}
\def\nconf{%
\renewcommand\stacktype{L}\mathbin{\ensurestackMath{%
  \ThisStyle{\stackon[0pt]{\SavedStyle\dwakola}{\SavedStyle/}}}}}
\newcommand{\grill}{\mathscr{G}}

\newcommand\mathbackslash{\raisebox{.4pt}{\texttt{/}}}
\def\notcon{% the separation relation
  \renewcommand\stacktype{L}\mathrel{\ensurestackMath{%
  \ThisStyle{\stackon[0pt]{\SavedStyle\con}{\SavedStyle\mathbackslash}}}}%
}
\let\separ=\notcon

\def\notconk{% the separation relation
  \renewcommand\stacktype{L}\mathrel{\ensurestackMath{%
  \ThisStyle{\stackon[0pt]{\SavedStyle\conk}{\SavedStyle\mathbackslash}}}}%
}

\def\notcond{% the separation relation
  \renewcommand\stacktype{L}\mathrel{\ensurestackMath{%
  \ThisStyle{\stackon[0pt]{\SavedStyle\cond}{\SavedStyle\mathbackslash}}}}%
}

\DeclareMathOperator{\upop}{\uparrow} %upper arrow operator
\DeclareMathOperator{\downop}{\downarrow} %lower arrow operator
\newcommand\twodownop{\raisebox{-1pt}{$\mathop{\rotatebox{90}{$\twoheadleftarrow$}}$}} %downward << closure operation
\newcommand\twoupop{\raisebox{-1pt}{$\mathop{\rotatebox{90}{$\twoheadrightarrow$}}$}} %upward << closure operation

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%---------------------------------Theories-------------------------------
\DeclareMathOperator{\Th}{Th} %theory of a model
\newcommand\PA{\mathsf{PA}} %first order Peano Arithmetic
\newcommand{\num}{\overline} %the numeral for a number
\newcommand{\godel}[1]{\ulcorner #1\urcorner} %godel number of an expression
\newcommand{\forces}{\Vdash} %forcing relation
\newcommand{\nforces}{\nVdash} %complement of forcing relation


%---------------------------------Topology-------------------------------

\DeclareMathOperator{\Cl}{Cl}
\DeclareMathOperator{\Int}{Int}
\newcommand\cl[1]{\overline{#1}}

\newcommand{\Basis}{\mathscr{B}} %basis for topology
\newcommand{\topo}{\mathscr{O}} %family of open sets
\newcommand{\topone}{\mathscr{O}^+} %family of non-empty open sets
\newcommand{\topoc}{\mathscr{C}} %family of closed sets

%---------------------------------Fonts---------------------------------------
\newcommand\calA{\mathcal{A}}
\newcommand\calB{\mathcal{B}}
\newcommand\calC{\mathcal{C}}
\newcommand\calD{\mathcal{D}}
\newcommand\calE{\mathcal{E}}
\newcommand\calF{\mathcal{F}}
\newcommand\calG{\mathcal{G}}
\newcommand\calH{\mathcal{H}}
\newcommand\calK{\mathcal{K}}
\newcommand\calL{\mathcal{L}}
\newcommand\calM{\mathcal{M}}
\newcommand\calN{\mathcal{N}}
\newcommand\calR{\mathcal{R}}
\newcommand\calS{\mathcal{S}}
\newcommand\calT{\mathcal{T}}
\newcommand\calU{\mathcal{U}}
\newcommand\calX{\mathcal{X}}
\newcommand\calY{\mathcal{Y}}

\newcommand\mfr{\mathfrak}
\newcommand\frA{\mfr{A}}
\newcommand\frB{\mfr{B}}
\newcommand\frD{\mfr{D}}
\newcommand\frF{\mfr{F}}
\newcommand\frH{\mfr{H}}
\newcommand\frI{\mfr{I}}
\newcommand\frK{\mfr{K}}
\newcommand\frL{\mfr{L}}
\newcommand\frM{\mfr{M}}
\newcommand\frN{\mfr{N}}
\newcommand\frO{\mfr{O}}
\newcommand\frP{\mfr{P}}
\newcommand\frQ{\mfr{Q}}
\newcommand\frR{\mfr{R}}
\newcommand\frU{\mfr{U}}


\newcommand{\frg}{\mfr{g}}
\newcommand{\frh}{\mfr{h}}
\newcommand{\frp}{\mfr{p}}
%\newcommand{\frq}{\mfr{q}}
\newcommand{\frr}{\mfr{r}}
\newcommand{\frs}{\mfr{s}}

\newcommand\mbf{\mathbf}
\newcommand\bfB{\mbf{B}}
\newcommand\bfC{\mbf{C}}
\newcommand\bfF{\mbf{F}}
\newcommand\bfG{\mbf{G}}
\newcommand\bfK{\mbf{K}}

\newcommand\mrm{\mathrm}

\newcommand\rmp{\mrm{p}}
\newcommand\rmq{\mrm{q}}

\newcommand\rmI{\mrm{I}}
\newcommand\rmM{\mrm{M}}
\newcommand\rmU{\mrm{U}}
\newcommand\rmT{\mrm{T}}

\newcommand{\scrA}{\mathscr{A}}
\newcommand{\scrB}{\mathscr{B}}
\newcommand{\scrC}{\mathscr{C}}
\newcommand{\scrD}{\mathscr{D}}
\newcommand{\scrE}{\mathscr{E}}
\newcommand{\scrF}{\mathscr{F}}
\newcommand{\scrG}{\mathscr{G}}
\newcommand{\scrH}{\mathscr{H}}
\newcommand{\scrI}{\mathscr{I}}
\newcommand{\scrJ}{\mathscr{J}}
\newcommand{\scrK}{\mathscr{K}}
\newcommand{\scrL}{\mathscr{L}}
\newcommand{\scrM}{\mathscr{M}}
\newcommand{\scrN}{\mathscr{N}}
\newcommand{\scrR}{\mathscr{R}}
\newcommand{\scrS}{\mathscr{S}}

%---------------------------------Relations----------------------------------------

\newcommand\mrel{\mathrel}
\newcommand\Rel{\mathrel{R}}
\newcommand\leqs{\leqslant}
\newcommand\geqs{\geqslant}

%---------------------------------Other----------------------------------------

\newcommand\seq[1]{\langle #1_n \rangle_{n \in \Nat}}
\newcommand\dftt{\mathtt{df}\,}
\newcommand{\dom}{\mathrm{dom}} %the domain of a structure, function etc.
\newcommand{\Tmax}{T_{\mathrm{max}}} %the set of maximal extension of a theory T


\newcommand\suchthat{\,\middle\vert\,} %abstraction operator

%rules of inference macro

\newcommand*{\inference}[3][t]{%
   \begingroup
   \def\and{\\}%
   \begin{tabular}[#1]{@{\enspace}c@{\enspace}}
   #2 \\
   \hline
   #3
   \end{tabular}%
   \endgroup
}







==> bbm-without-txfonts.tex <==
\makeatletter
\DeclareSymbolFont{lettersA}{U}{txmia}{m}{it}
\SetSymbolFont{lettersA}{bold}{U}{txmia}{bx}{it}
\DeclareFontSubstitution{U}{txmia}{m}{it}

\DeclareMathSymbol{\m@thbbch@rA}{\mathord}{lettersA}{129}
\DeclareMathSymbol{\m@thbbch@rB}{\mathord}{lettersA}{130}
\DeclareMathSymbol{\m@thbbch@rC}{\mathord}{lettersA}{131}
\DeclareMathSymbol{\m@thbbch@rD}{\mathord}{lettersA}{132}
\DeclareMathSymbol{\m@thbbch@rE}{\mathord}{lettersA}{133}
\DeclareMathSymbol{\m@thbbch@rF}{\mathord}{lettersA}{134}
\DeclareMathSymbol{\m@thbbch@rG}{\mathord}{lettersA}{135}
\DeclareMathSymbol{\m@thbbch@rH}{\mathord}{lettersA}{136}
\DeclareMathSymbol{\m@thbbch@rI}{\mathord}{lettersA}{137}
\DeclareMathSymbol{\m@thbbch@rJ}{\mathord}{lettersA}{138}
\DeclareMathSymbol{\m@thbbch@rK}{\mathord}{lettersA}{139}
\DeclareMathSymbol{\m@thbbch@rL}{\mathord}{lettersA}{140}
\DeclareMathSymbol{\m@thbbch@rM}{\mathord}{lettersA}{141}
\DeclareMathSymbol{\m@thbbch@rN}{\mathord}{lettersA}{142}
\DeclareMathSymbol{\m@thbbch@rO}{\mathord}{lettersA}{143}
\DeclareMathSymbol{\m@thbbch@rP}{\mathord}{lettersA}{144}
\DeclareMathSymbol{\m@thbbch@rQ}{\mathord}{lettersA}{145}
\DeclareMathSymbol{\m@thbbch@rR}{\mathord}{lettersA}{146}
\DeclareMathSymbol{\m@thbbch@rS}{\mathord}{lettersA}{147}
\DeclareMathSymbol{\m@thbbch@rT}{\mathord}{lettersA}{148}
\DeclareMathSymbol{\m@thbbch@rU}{\mathord}{lettersA}{149}
\DeclareMathSymbol{\m@thbbch@rV}{\mathord}{lettersA}{150}
\DeclareMathSymbol{\m@thbbch@rW}{\mathord}{lettersA}{151}
\DeclareMathSymbol{\m@thbbch@rX}{\mathord}{lettersA}{152}
\DeclareMathSymbol{\m@thbbch@rY}{\mathord}{lettersA}{153}
\DeclareMathSymbol{\m@thbbch@rZ}{\mathord}{lettersA}{154}

\long\def\DoLongFutureLet #1#2#3#4{%
   \def\@FutureLetDecide{#1#2\@FutureLetToken
      \def\@FutureLetNext{#3}\else
      \def\@FutureLetNext{#4}\fi\@FutureLetNext}
   \futurelet\@FutureLetToken\@FutureLetDecide}
\def\DoFutureLet #1#2#3#4{\DoLongFutureLet{#1}{#2}{#3}{#4}}
\def\@EachCharacter{\DoFutureLet{\ifx}{\@EndEachCharacter}%
   {\@EachCharacterDone}{\@PickUpTheCharacter}}
\def\m@keCharacter#1{\csname\F@ntPrefix#1\endcsname}
\def\@PickUpTheCharacter#1{\m@keCharacter{#1}\@EachCharacter}
\def\@EachCharacterDone \@EndEachCharacter{}

\DeclareRobustCommand*{\varmathbb}[1]{\gdef\F@ntPrefix{m@thbbch@r}%
  \@EachCharacter #1\@EndEachCharacter}
\makeatother


